LTIatCMU at SemEval-2020 Task 11: Incorporating Multi-Level Features for Multi-Granular Propaganda Span Identification

In this paper we describe our submission for the task of Propaganda Span Identification in news articles. We introduce a BERT-BiLSTM based span-level propaganda classification model that identifies which token spans within the sentence are indicative of propaganda. The "multi-granular" model incorporates linguistic knowledge at various levels of text granularity, including word, sentence and document level syntactic, semantic and pragmatic affect features, which significantly improve model performance, compared to its language-agnostic variant. To facilitate better representation learning, we also collect a corpus of 10k news articles, and use it for fine-tuning the model. The final model is a majority-voting ensemble which learns different propaganda class boundaries by leveraging different subsets of incorporated knowledge and attains $4^{th}$ position on the test leaderboard. Our final model and code is released at https://github.com/sopu/PropagandaSemEval2020.

==> sections/data.tex <==
\section{Corpus Description}
\label{sec:data}

==> sections/discussion.tex <==
\section{Discussion}
\label{sec:discussion}

==> sections/experiments.tex <==
%\section{Experimental Setup}
%\label{sec:experiments}
%
%
%
%\subsection{Evaluation Metric}
%\label{sec:eval_metric}


==> sections/related_work.tex <==
\section{Related work}
\label{sec:related_work}
The original paper of \cite{propaganda-emnlp-2019} frames the task as multi-granular classification wherein they experiment with several neural architectures using different variants of BERT \cite{bert-devlin-2019}. In their work, they use a fine tuned BERT to perform a 19 way classification (18 for propaganda techniques and 1 for None) on a token level and use the CLS token for binary classification to detect whether the sentence has any propaganda spans or not. They experiment with joint training and using the sentence embedding as granularity. We take inspiration from their Multi-Granular network in which they use the predictions from the sentence level task to influence the predictions of the span level task. We use the Multi-Granular network as a baseline for our model. %However we refer only to the Multi-Granularity network, which we use as a baseline. 

% \noindent\textbf{(a) BERT: } 
% They append a linear layer to the pre-trained BERT model of \citet{bert-devlin-2019} and  fine-tune it. They use the hidden representation of the final layer for the word embedding and perform a 19 way classification (for the 18 different propaganda techniques and None). Likewise they use the CLS token to represent the sentence and perform binary classification to detect whether the sentence was propaganda or not. 

% \noindent\textbf{(b) BERT-Joint: } They perform joint training of both the sentence and the word embeddings for their respective task of sentence and span level classification. 

% \noindent\textbf{(c) BERT-Granu: } They append the learnt sentence embedding along with the word embedding to identify spans of propaganda. This enables the words to gain additional contextual information from the sentence. 



% \noindent \textbf{(d) Mult-Granular Network:} In this architecture, they leverage the predictions from the sentence level classification task and use it to modify the prediction scores for the span-based classification task.  Specifically, they multiply the predicted score for the propaganda classes along with the sentence score (probability of a sentence being propagandist). This ensures that the softmax probability of a word belonging to a particular class remains the same but the final cross-entropy loss is influenced more by sentences which are more strongly detected as propagandist. 

% These multi-granularity BERT neural architecture serves as the baseline for this task.

Some of the prior work from the first shared task \cite{shared-task-findings-2019} sheds some insights on the propaganda detection task. Specifically, 
the team \textbf{newspeak} \cite{fine-tune-bert-propaganda} achieved the highest performance on fragment level classification by fine-tuning BERT. They also over-sampled the under-represented classes using curriculum learning. 
The team \textbf{Stalin } \cite{synthetic-prop-embeddings}
% addressed the issues of data scarcity and the overhead of fine-tuning embeddings through data-augmentation and generating additional synthetic contextualized embeddings. They 
used pre-trained models like BERT \cite{bert-devlin-2019}, ELMO \cite{elmo-2018} and GROVER \cite{Grover-2109} to generate contextual embeddings and oversample using SMOTE \cite{chawla2002smote} to generate synthetic representations, which are further fine-tuned. %for each token annotated with different propaganda techniques. To ensure all classes have the same representation, oversampling is carried out using SMOTE \cite{chawla2002smote} to generate synthetic embeddings. 
%These synthetic embeddings are further fine-tuned using simple neural layers like (linear layer with ReLU activation and/or Bi-LSTM) followed by a softmax layer over the 19 classes.  
The team \textbf{MIC-CIS} \cite{linguistic-features-prop} leveraged additional information like linguistic features (POS-TAGs, NER, readability scores, sentiment, emotion etc.), topical information of the document, different embedding representations like FastText and BERT, and finally performed an ensemble. Unlike the previous models which treated the task as classification, they performed sequence tagging using Bi-LSTM and CRF with Multi-tasking. Our work is most similar to theirs, except that we make use of multi-granular BERT, incorporate features from multiple levels and don't perform sequence tagging using CRF. %(namely predicting whether a token was propagandist and if so, which type of propaganda). 
In a similar fashion, the team \textbf{CUNLP} \cite{uby-embeddings-propaganda} builds upon the flair framework \citet{flair} by combining character and word embeddings (pre-trained GloVe embeddings and pre-trained Word2vec embeddings  on Urban dictionary\footnote{\url{https://data.world/jaredfern/urban-dictionaryembeddin}} ) and passes it through a BiLSTM-CRF model. They also incorporate additional features like LIWC \cite{liwc} and UBY embeddings \cite{uby-2012}. 


% \begin{table}[h]
%     \centering
%     \begin{tabular}{l|c|c|c}
%       \textbf{Approach}& \textbf{F1-score}& \textbf{Precision}&\textbf{Recall}\\ \hline
%          Multi-Granu&  0.2442& 0.2105&\textbf{ 0.2258} \\
%          newspeak&\textbf{0.2488}& 0.2862& 0.2200\\
%          MIC-CIS& 0.1998 &0.2234& 0.1808\\
%          Stalin&0.1453& 0.1920& 0.1169 \\
%          CUNLP&0.1311 &\textbf{0.3234}& 0.0822\\
%     \end{tabular}
%     \caption{Results of the Fragment Level Classification of the related baselines.\todo{from where are these taken / generated?}}
%     \label{tab:propaganda-table}
% \end{table}

% We present the results of the fragment level classification task of the proposed methods in Table \ref{tab:propaganda-table}. 
%It is to be noted that the current SemEval 2020 Task 11 has framed the problem in a slightly different fashion. The first task is to identify spans of propagandist content in an article while the second task entails identifying the type of propaganda in a given span. For this particular project and the SemEval competition, we focus on the first task. 
%In addition to the ideas proposed by prior work, that shows that using linguistic features helps the performance, we incorporate syntactic features as well, on a multi-level fashion, namely word, sentence and document level.
%We also collect a large corpus of about 10k news articles to fine-tune BERT. 
% \subsection{Proposed Approach}
% Our proposed approach includes the following ideas or steps. 

% (i) Pre-train BERT on a large collection of news articles collected from different sources. To ensure equal representation, we scraped approximately 10k articles from propaganda websites like Lew Rockwell, \footnote{\url{https://www.lewrockwell.com/}} Vdare\footnote{\url{https://vdare.com/}}, and SHTFplan.com \footnote{\url{http://www.shtfplan.com/}}, and another 10k articles from trusted non-propagandist sources like CNN \footnote{\url{https://www.cnn.com/}} and New York Times\footnote{\url{https://www.nytimes.com/}}. We scraped articles spanning 2018 and mid of 2019 to ensure that the articles follow the same topical distribution as that of the training articles. 

% (ii) To address the scarcity of data, we intend to perform data-augmentation using self-training. Specifically, we will use our intermediate trained model to predict spans of propagandist content amongst the scraped unlabelled data. We perform thresholding to select the top candidate spans, which are subsequently treated as gold labels. We then augment the new labels to the original data and repeat the procedure till there is no significant improvement in performance.  Further, to address the issue of imbalance of propaganda spans vs non-propaganda spans, we experiment with different weighing strategies.

% (iii) We also hope to improve upon the proposed multi-granularity network. We will incorporate additional linguistic and lexical features associated with each word such as LIWC \cite{liwc}, Empath \cite{fast2016empath}, propaganda score \footnote{Ratio of probability of a word being in propaganda spans to the probability of the word in non-propaganda spans}, NER, and POS tags. We will append syntactic information by representing the path from a word to the root in its constituent parse tree as a 30 dimensional embedding. Furthermore, we seek to leverage additional document context while classifying a sentence as propaganda. 
